Network Coding-Based Link Failure Recovery over Large Arbitrary Networks

Network coding-based link failure recovery techniques provide near-hitless recovery and offer high capacity efficiency. Diversity coding is the first technique to incorporate coding in this field and is easy to implement over small arbitrary networks. However, its capacity efficiency is restricted by its systematic coding and high design complexity even though it has lower complexity than the other coding-based recovery techniques. Alternative techniques mitigate some of these limitations, but they are difficult to implement over arbitrary networks. In this paper, we propose a novel non-systematic coding technique and a simple design algorithm to implement the diversity coding-based (or network coding-based) recovery over arbitrary networks. The design framework consists of two parts. An ILP formulation for each part is developed. The simulation results suggest that both the novel coding structure and the novel design algorithm lead to higher capacity efficiency for near-hitless recovery. The new design algorithm is able to achieve optimal results in large arbitrary networks.

==> algorithm2e/algorithm2e_ex01.tex <==
\SetAlgoVlined
\eIf{cond1}{
  a line\;
  a line\;
}{
  another line\;
  another line\;
}


==> algorithm2e/algorithm2e_ex02.tex <==
\SetAlgoNoLine
\If{cond2}{
  second if\;
  second if\;
}


==> algorithm2e/algorithm2e_ex03.tex <==
\lIf{cond3}{ another example}
\Else{
  a block\;
  a block\;
}


==> algorithm2e/algorithm2e_ex04.tex <==
\lIf{cond4}{ok} \lElse{wrong}\;

==> algorithm2e/algorithm2e_ex05.tex <==
\SetAlgoVlined
\lIf{cond5}{cond5 true}\;
\uElseIf{cond51}{
  cond 5 false\;
  but cond51 true\;
}
\ElseIf{}{
  all is wrong\;
  \Return result52\;
}


==> algorithm2e/algorithm2e_ex06.tex <==
\SetAlgoLined
\uIf{cond6}{
  cond6 is ok\;
  always ok\;
}
\uElseIf{cond62}{
  choose result62\;
  \Return result62\;
}
\Else{
  all is wrong\;
  do something else\;
}


==> algorithm2e/algorithm2e_ex07.tex <==
Let's have a look at what we can do
with if-then-else and side comments\;
\eIf{if-then-else test}{
  no comment here\;
  neither in then\;
}{
  nor in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  then with a comment\;
}(\tcc*[f]{comment in else})
{
  here we are in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  again a comment in then\;
}{
  but not in else\;
}
\eIf{if-then-else test}{
  this time, no comment in then\;
}(\tcc*[f]{else comment})
{
  but one comment in else\;
}
Let's try with other if possibilities\;
\lIf(\tcc*[h]{lif comment}){test}{text}
\uIf(\tcc*[f]{uif comment}){test}{
  then text\;
}
\uElseIf(\tcc*[f]{comment}){test}{
  elseif text\;
}
\lElseIf(\tcc*[h]{comment}){test}{text}
\lElse(\tcc*[f]{comment}){text}


==> algorithm2e/algorithm2e_exAlgoDisjdecomp.tex <==
\IncMargin{1em}
\begin{algorithm}
  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}

  \Input{A bitmap $Im$ of size $w\times l$}
  \Output{A partition of the bitmap}
  \BlankLine
  \emph{special treatment of the first line}\;
  \For{$i\leftarrow 2$ \KwTo $l$}{
    \emph{special treatment of the first element of line $i$}\;
    \For{$j\leftarrow 2$ \KwTo $w$}{\label{forins}
      \Left$\leftarrow$ \FindCompress{$Im[i,j-1]$}\;
      \Up$\leftarrow$ \FindCompress{$Im[i-1,]$}\;
      \This$\leftarrow$ \FindCompress{$Im[i,j]$}\;
      \If(\tcp*[h]{O(\Left,\This)==1}){\Left compatible with \This}{\label{lt}
        \lIf{\Left $<$ \This}{\Union{\Left,\This}}\;
        \lElse{\Union{\This,\Left}\;}
      }
      \If(\tcp*[f]{O(\Up,\This)==1}){\Up compatible with \This}{\label{ut}
        \lIf{\Up $<$ \This}{\Union{\Up,\This}}\;
        \tcp{\This is put under \Up to keep tree as flat as possible}\label{cmt}
        \lElse{\Union{\This,\Up}}\tcp*[r]{\This linked to \Up}\label{lelse}
      }
    }
    \lForEach{element $e$ of the line $i$}{\FindCompress{p}}
  }
  \caption{disjoint decomposition}\label{algo_disjdecomp}
\end{algorithm}\DecMargin{1em}

==> algorithm2e/algorithm2e_exIR.tex <==
\begin{algorithm}
\DontPrintSemicolon
\KwData{$G=(X,U)$ such that $G^{tc}$ is an order.}
\KwResult{$G'=(X,V)$ with $V\subseteq U$ such that $G'^{tc}$ is an
interval order.}
\Begin{
  $V \longleftarrow U$\;
  $S \longleftarrow \emptyset$\; 
  \For{$x\in X$}{ 
    $NbSuccInS(x) \longleftarrow 0$\;
    $NbPredInMin(x) \longleftarrow 0$\;
    $NbPredNotInMin(x) \longleftarrow |ImPred(x)|$\;
    }
  \For{$x \in X$}{
    \If{$NbPredInMin(x) = 0$ {\bf and} $NbPredNotInMin(x) = 0$}{
      $AppendToMin(x)$}
    } 
    \nl\While{$S \neq \emptyset$}{\label{InRes1}
    \nlset{REM} remove $x$ from the list of $T$ of maximal index\;\label{InResR}
    \lnl{InRes2}\While{$|S \cap  ImSucc(x)| \neq |S|$}{ 
      \For{$ y \in  S-ImSucc(x)$}{
        \{ remove from $V$ all the arcs $zy$ : \}\;
        \For{$z \in  ImPred(y) \cap  Min$}{
          remove the arc $zy$ from $V$\;
          $NbSuccInS(z) \longleftarrow NbSuccInS(z) - 1$\;
          move $z$ in $T$ to the list preceding its present list\;
          \{i.e. If $z \in T[k]$, move $z$ from $T[k]$ to 
           $T[k-1]$\}\;
          }
        $NbPredInMin(y) \longleftarrow 0$\;
        $NbPredNotInMin(y) \longleftarrow 0$\;
        $S \longleftarrow S - \{y\}$\;
        $AppendToMin(y)$\;
        }
      }
    $RemoveFromMin(x)$\;
    }
  }  
\caption{IntervalRestriction\label{IR}}
\end{algorithm}


==> algorithm2e/algorithm2e_exfor.tex <==
\SetAlgoLined
\ForAll{elements of $S_1$}{
  remove an element e from $S_1$\;
  put e in the set $S_2$\;
  }
\lFor{i=1 \emph{\KwTo}max}{mark i}\;
\ForEach{$e$ in the set}{
  put $e$ in ${\cal E}$\;
  mark $e$\;
}


==> algorithm2e/algorithm2e_exrepeat.tex <==
\Repeat{this stop condition}{
  the text of the loop\;
  another line\;
  always in the loop\;
  }
\lRepeat{stop}{a one line loop}


==> algorithm2e/algorithm2e_exswitch.tex <==
\Switch{the value of T}{
  \uCase{a value}{
    do this\;
    do that\;
  }
  \lCase{another value}{one line}\;
  \Case{last value}{
    do this\;
    break\;
  }
  \Other{
    for the other values\;
    do that\;
  }
}

